A Tutorial on Design Obfuscation: from Transistors to Systems

The recent advances in the area of design obfuscation are encouraging, but may present themselves as hard to read for a non-specialist audience. This tutorial uncovers these advances in a clear language, contrasting the approaches that can be implemented at layout level, in the netlist of a circuit, or even at chip level. This tutorial also highlights the available support, both from the tooling side and the logistics of fabricating an obfuscated integrated circuit.

==> acronyms.tex <==
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{flop}{FLOP}{FLoating-point Operations Per Second}
\newacronym{asild}{ASIL-D}{Automotive Safety Integrity Level D}
\newacronym{sdc}{SDC}{Single Data Corruption}
\newacronym{secded}{SECDED}{Single Error Correction Double Error Detection}
\newacronym{dmr}{DMR}{Double Modular Redundancy}
\newacronym{fit}{FIT}{Failure In Time}
\newacronym{kvf}{KVF}{Kernel Vulnerability Factor}
\newacronym{adas}{ADAS}{Advanced Driver Assistance Systems}
\newacronym{hog}{HOG}{Histogram of Oriented Gradients}
\newacronym{yolo}{YOLO}{You Only Look Once}
\newacronym{ecc}{ECC}{Error Correction Code}
\newacronym{hpc}{HPC}{High Performance Computing}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym[\glslongpluralkey={Bounding Boxes}]{bb}{BB}{Bounding Box}
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{lvf}{LVF}{Layer Vulnerability Factor}
\newacronym{relu}{ReLU}{Rectified Linear Units}
\newacronym{ann}{ANN}{Artificial Neural Network}
\newacronym{pvf}{PVF}{Program Vulnerability Factor}
\newacronym{avf}{AVF}{Architecture Vulnerability Factor}
\newacronym{tmr}{TMR}{Tiple Modular Redundancy}
\newacronym{rf}{RF}{Register File}
\newacronym{inst}{INST}{Instruction}

